Multi-Commodity Flow with In-Network Processing

Modern networks run "middleboxes" that offer services ranging from network address translation and server load balancing to firewalls, encryption, and compression. In an industry trend known as Network Functions Virtualization (NFV), these middleboxes run as virtual machines on any commodity server, and the switches steer traffic through the relevant chain of services. Network administrators must decide how many middleboxes to run, where to place them, and how to direct traffic through them, based on the traffic load and the server and network capacity. Rather than placing specific kinds of middleboxes on each processing node, we argue that server virtualization allows each server node to host all middlebox functions, and simply vary the fraction of resources devoted to each one. This extra flexibility fundamentally changes the optimization problem the network administrators must solve to a new kind of multi-commodity flow problem, where the traffic flows consume bandwidth on the links as well as processing resources on the nodes. We show that allocating resources to maximize the processed flow can be optimized exactly via a linear programming formulation, and to arbitrary accuracy via an efficient combinatorial algorithm. Our experiments with real traffic and topologies show that a joint optimization of node and link resources leads to an efficient use of bandwidth and processing capacity. We also study a class of design problems that decide where to provide node capacity to best process and route a given set of demands, and demonstrate both approximation algorithms and hardness results for these problems.

==> makefile <==
RCSFLAGS= -l
MAIN= main
FINAL= final
TEXPARTS= 
BIBPARTS= BIB/*.bib
FIGPARTS= FIG/*.png

OTHER= mkfinal.pl makefile
ALL= $(MAIN).tex $(TEXPARTS) $(BIBPARTS) $(FIGPARTS) $(OTHER)

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS)
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

final: $(FINAL).pdf

$(FINAL).pdf: $(MAIN).tex mkfinal.pl
	mkfinal.pl $(MAIN).tex > $(FINAL).tex
	pdflatex $(FINAL).tex
	bibtex $(FINAL)
	pdflatex $(FINAL).tex
	pdflatex $(FINAL).tex

try: $(MAIN).tex
	pdflatex $(MAIN)

clean:
	\rm -f *.dvi $(MAIN).ps $(MAIN).pdf *.bbl *.aux *.log *.blg *.toc all.tar* uu \
	*~ *.bak *.lbl *.brf *.out *.synctex.gz

spotless: clean
	\rm -f $(MAIN).ps $(MAIN).pdf
	\rm -f $(FINAL).*
	\rm -rf TST

all.tar:
	tar cvfh all.tar $(ALL)

